A Passivity-Based Variable Impedance Controller for Incremental Learning of Periodic Interactive Tasks

In intelligent manufacturing, robots are asked to dynamically adapt their behaviours without reducing productivity. Human teaching, where an operator physically interacts with the robot to demonstrate a new task, is a promising strategy to quickly and intuitively reconfigure the production line. However, physical guidance during task execution poses challenges in terms of both operator safety and system usability. In this paper, we solve this issue by designing a variable impedance control strategy that regulates the interaction with the environment and the physical demonstrations, explicitly preventing at the same time passivity violations. We derive constraints to limit not only the exchanged energy with the environment but also the exchanged power, resulting in smoother interactions. By monitoring the energy flow between the robot and the environment, we are able to distinguish between disturbances (to be rejected) and physical guidance (to be accomplished), enabling smooth and controlled transitions from teaching to execution and vice versa. The effectiveness of the proposed approach is validated in wiping tasks with a real robotic manipulator.

==> sections/exp_control.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm,clip,width=\textwidth, height=7.5cm]{images/VS-CF_VS-VF_new.pdf}
    %\vspace{-.5cm}
    \caption{Results of the ultrasound experiment on a dummy chest in nominal conditions. (left) VS-CF, (right) VS-VF. The results of the CS and CF controllers are not reported here for the sake of space. A video of the experiments is available in the multimedia extension and in \url{https://youtu.be/IwQhgzcd4IM}.}
    \label{fig:vs_comparison}
    %\vspace{-2mm}
\end{figure*}
\begin{figure*}[!ht]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm,clip,width=\textwidth, height=7.5cm]{images/comparison_disturb_new.pdf}
    %\vspace{-.5cm}
    \caption{Comparison of ultrasound experiment on a dummy chest with disturbances: (a) VS-VF, (b) CS, (c) CF. }
    \label{fig:comparison_dist}
    %\vspace{-4mm}
\end{figure*}

We compare the behaviour of the \textit{CF} and \textit{CS} controller against \textit{VS}-\textit{CF} and \textit{VS}-\textit{VF} that exploit the information of the body
reconstruction. For simplicity, we assume that the value of the rotational stiffness is constant in each direction. The optimisation variable $\boldsymbol{K}^d$ is then a diagonal $3$x$3$ matrix, where each element represents the stiffness in one direction. The minimum and maximum stiffness are identical in every direction and respectively equal to $K_{i,i}^{min}=\SI{100}{N/m}$ and $K_{i,i}^{max}=\SI{1000}{N/m}$.
The inner PD force controller gains, that ensures the force tracking as explained in in~\cite{scherzinger2017forward}, were set to
$k_p = 0.3$ and $k_d = 0.01$ for all the controllers beside the
\textit{CS} where we let the default values of $k_p = 0.05$ and
$k_d = 0.0005$ due to instability problems. 
For experiments, a
reference target is maintained at constant $z$ under the surface of
the dummy to ensure contact and is moved with constant velocity of
$\SI{1}{\centi\meter\cdot\second^{-1}}$ in the longitudinal direction
of the chest dummy. Note that the force controller is hybrid since the
$x$ and $y$ axes are controlled by the compliant controller, while the
$z$ axis is controlled in force, hence it is not possible to give a
reference value to this axis. As expected, the force generated by the
\textit{CS} control is strongly dependent on the shape of the body
(\autoref{fig:comparison_dist}: when the surface is further from
the target, the generated force is stronger than when the surface is
closer. The force controller, instead, can track the target force
without any problem but has the downside that it cannot be controlled
in position, so it is not possible to raise the end-effector from the
surface as in the case of the end of the experiment. Also, in the case of
problems, it would not be possible to stop the end effector except by
resetting the target force it has to reach, which may result in
dangerous motions. The \textit{VS}-\textit{CF} control can track a
reference force as good as a force control
(\autoref{fig:vs_comparison}), but without its downsides. It is
possible to control all the axes when in free motion and also to
suddenly detach the end-effector from the surface in case of
necessity. On top, it uses the information registered by the
reconstruction to cut the reference force when the maximum penetration
is reached preventing the tip from sinking further. The
\textit{VS}-\textit{VF}, instead of tracking a constant force, it is
tracking the force necessary to keep a constant penetration
into the material. In this case, the minimum force avoids pushing too
hard on the stiff points, such as the ribs: at these points,
to achieve the desired penetration, it would require more force than
the maximum force we want to impart on the body.

The same test is done under the action of some disturbances to
demonstrate the inherent safety of this new approach
(\autoref{fig:comparison_dist}). The disturbance consists in raising the dummy to see how the different controls would handle the situation. Given that the
safety of the approaches \textit{VS}-\textit{CF} and
\textit{VS}-\textit{VF} is identical, indeed both use energy tanks and
energy valves to avoid the creation of sudden forces, this test was
done on one of them. We decided to choose the second one given that, in
this approach, the maximum force is limited by a constant. Instead, in
the first approach, the maximum force limit can be subject to
estimation errors leaving room for possible dangerous
behaviour. \autoref{fig:comparison_dist} shows that, as soon as the
end-effector starts to be moved away, the stiffness of the impedance
spring starts decreasing until no force is acting anymore; then, the
spring value is limited to its minimum until the moment of the new
contact. At the moment of contact, the stiffness would suddenly increase, but the presence of the valves partially limits its
growth and restricts the tank from being emptied too quickly.

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=0cm 2cm 23cm 0cm,clip,width=\columnwidth]{images/VS-VF_dist.pdf}
%     \vspace{-.8cm}
%     \caption{Results of ultrasound experiment on a dummy chest with disturbances (VS-VF).}
%     \label{fig:vs_vf_dist}
%     \vspace{-3mm}
% \end{figure}




==> sections/exp_params.tex <==
% \noindent - Evaluation of the procedure: plot with convergence \\
% - Evaluation of the  parameters: table with MSE (load/unload), plot of one load test, comparison between measured force and estimated with parameters \\
% - Plot of the smooth surface obtained with the GP \\
\begin{figure}[t!]
    \centering
    % \includegraphics[trim=0cm 1cm 0cm 3cm,clip,width=\columnwidth]{images/load_cycle_new.pdf}
    \begin{tikzpicture}
    [spy using outlines={lens={scale=2,rotate=-16}, ellipse, size=2.5cm, height=1.5cm, connect spies},
    ]
        \node[inner sep=0pt] (robot) at (0,0) {\includegraphics{images/comparison.pdf}};
    
        \spy [red] on (0.4,0) in node [left,lens={scale=2,rotate=2},rotate=16] at (4,0.2);

    \end{tikzpicture}
    %\includegraphics[trim=0cm 0cm 0cm 4.5cm,clip,width=\columnwidth]{images/load_cycle_new.pdf}
    %{images/ciclodicarico.eps}
    %\vspace{-.8cm}
    \caption{Load tests obtained with the different models.}
    \label{fig:loadcycle}
    %\vspace{-3mm}
\end{figure}
The standard procedure to evaluate a viscoelastic model is to perform a load and unload test at constant velocity. This test is done with a Cartesian position controller in the following way: the loading phase is done with constant velocity of $\SI{3}{\centi\meter\cdot\second^{-1}}$ for $\SI{0.75}{\second}$, the load is maintained then for $\SI{10}{\second}$ to reach the equilibrium and finally there is the unloading phase with a velocity of $\SI{1.5}{\centi\meter\cdot\second^{-1}}$ for $\SI{1.5}{\second}$. Results of this test in \autoref{fig:loadcycle} show the limitation of the linear Kelvin-Voight, i.e., for the first phase of the penetration the model prediction is far from the measured force. The Hunt-Crossley model achieves better results in imitating how the body react under a load. 
In \autoref{tab:model_residuals} are shown the residual of the least square \autoref{eq:sm} when varying $\beta$. Minimising the value of this variable over different points of the puppet we obtain that $\beta=1.35$ is the best compromise.
%In \autoref{fig:loadtime} is shown how the model behave over the time during the loading and unloading phase. 
%\begin{figure}[ht!]
%     \centering
%     \includegraphics[scale=0.4]{images/caricotempo.eps}
%     \caption{Prediction of the Hunt-Crossley model ($\beta=1.35$) compared with the force sensor during the loading cycle.}
%     \label{fig:loadtime}
% \end{figure}
This value of $\beta$ is used to estimate elasticity and viscosity of
the tissue with the sinusoidal palpation and the least square
method. A known issue of the least square method is that is crucial to
have a large amount of observations in order to retrieve precise
estimates. \autoref{fig:residuals} shows how the residuals are
affected by the palpation time; they decrease with exponential behaviour. We choose $\SI{5}{\second}$ as trade-off between length and precision of the estimation.
\begin{figure}[t!]
    \centering
    %\includegraphics[width=\columnwidth, height=3cm]{images/residuals.pdf}
    \includegraphics{images/residuals.pdf}
    %\vspace{-.5cm}
    \caption{Variation of residual as palpation time changes.}
    \label{fig:residuals}
    %\vspace{-4mm}
\end{figure}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[scale=0.4]{images/palpation.eps}
%     \caption{Results from the estimation of the parameters of the Cross Huntley model after $\SI{5}{\second}$ of plapation.}
%     \label{fig:palpation}
% \end{figure}
% \begin{table}[t]
% \begin{center}
% \begin{tabular}{|l|l|}
% \toprule
%   Model& Relative Residual Value \\ \hline
%   \midrule
%   Kelvin-Voight&  0.066\\ \hline
%  Hunt-Crossley $\beta$ = 1.5 &  0.029\\ \hline
%  Hunt-Crossley $\beta$ = 1.35&  0.014\\ \hline
%   Hunt-Crossley $\beta$ = 1.1 &  0.045 \\
% \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:model_residuals}
% \end{table}
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.2}
% \caption{Viscoelastic Model Validation}
% %\begin{adjustbox}{width=0.7\columnwidth,center}
% \centering
%     \begin{tabular}{l c c}
%     \toprule
%     \multicolumn{2}{c}{\textbf{Relative Residual Value (N)}}\\
%         \midrule
%         Kelvin-Voight&  0.066\\ 
%         Hunt-Crossley $\beta$ = 1.5 &  0.029\\ 
%         Hunt-Crossley $\beta$ = 1.35&  0.014\\ 
%         Hunt-Crossley $\beta$ = 1.1 &  0.045 \\
%         \bottomrule
%     \end{tabular}
%    % \end{adjustbox}
% \label{tab:model_residuals}
% \vspace{-3mm}
% \end{table}
The palpations on the chest dummy were made at a distance of $\SI{1}{\centi\meter}$ apart so that the surface could be accurately reconstructed. %There are methods such as in \cite{Chalasani2016ConcurrentPalpation} that test the points on the surface where the variance is greater in order to minimise the number of observations taken. In this case, they were not applied because we want to emphasise the usefulness of these data in the control strategy. 
\begin{figure}[t!]
    \centering
    % \includegraphics[trim=0cm 8cm 0cm 0cm,clip,width=\columnwidth]{images/map.eps}
    \includegraphics[width=\columnwidth]{images/map2.pdf}
    %\vspace{-.5cm}
    \caption{Resulting maps from the GPR computing the values of elasticity and viscosity every $\SI{0.1}{\milli\meter}$.}
    \label{fig:stiffdamp_map}
    %\vspace{-5mm}
\end{figure}
\begin{figure}[t!]
    \centering
    %\includegraphics[scale=0.4, height=5cm]{images/rec.pdf}
    %\vspace{-.5cm}
    \input{sections/reconstruction}
    \caption{Surface reconstruction with elasticity information. The view is rotated of \SI{180}{\degree} degrees wrt \autoref{fig:stiffdamp_map}  to better show the shape of the body.}
    \label{fig:surface}
    %\vspace{-3mm}
\end{figure}

In \autoref{fig:stiffdamp_map} are shown the elasticity and viscosity map computed using the GPR. Focussing on the elasticity map, it can be seen that there are 4 yellow lines, three more evident, and one less; those lines represent the ribs of the chest dummy that are stiffer than the rest of the surface. In \autoref{fig:surface} the dummy-specific elasticity map is projected on the surface reconstructed with the \texttt{GRIDFIT} algorithm. The upward tilt in the bottom left of the figure is the beginning of the shoulder that can be seen in \autoref{fig:setup}. It is interesting to notice that the rib covered by the pectoral muscle seems less stiff than the others covered only by a thin layer of skin.

\begin{table}[t!]
\renewcommand{\arraystretch}{1.2}
\caption{Viscoelastic Model Validation}
%\vspace{-2mm}
\centering
    \begin{tabular}{l c c c}
    \toprule
\multicolumn{4}{c}{\sc{Relative Residual Value [N]}}\\
        \midrule
        Kelvin-Voight& \multicolumn{3}{c}{Hunt-Crossley}\\
        & $\beta$ = 1.5 & $\beta$ = 1.35 & $\beta$ = 1.1 \\ 
        \cline{2-4} 
        0.066 & 0.029 & 0.014 & 0.045 \\
        \bottomrule
    \end{tabular}
\label{tab:model_residuals}
%\vspace{-4mm}
\end{table}






==> sections/problem.tex <==
\noindent 
- Description of the problem;\\
- Physical model + image of the model;\\
- Issues which might arise (exertion of high forces, assistance)

%involuntary patient movements during scanning; ii) inevitable errors in scan trajectory to patient registration; iii) highly-deformable skin surface difficult to be measured preoperatively 

==> sections/reconstruction.tex <==
\begin{tikzpicture}
\node[inner sep=0pt] (rec) at (0,0)
    {\includegraphics{images/rec.pdf}};
\node[right of = rec, color = red, xshift = 1.2cm, yshift=2cm](ribs){Ribs};
\draw[-latex, color = red] (ribs.west)--(-1.7,1){};
\draw[-latex, color = red] (ribs.west)--(-0.8,1.4){};
\draw[-latex, color = red] (ribs.west)--(0,1.2){};
\draw[-latex, color = red] (ribs.west)--(0.8,1.2){};
\end{tikzpicture}
